In Anticipation of Perfect Deepfake: Identity-anchored Artifact-agnostic Detection under Rebalanced Deepfake Detection Protocol

As deep generative models advance, we anticipate deepfakes achieving "perfection"-generating no discernible artifacts or noise. However, current deepfake detectors, intentionally or inadvertently, rely on such artifacts for detection, as they are exclusive to deepfakes and absent in genuine examples. To bridge this gap, we introduce the Rebalanced Deepfake Detection Protocol (RDDP) to stress-test detectors under balanced scenarios where genuine and forged examples bear similar artifacts. We offer two RDDP variants: RDDP-WHITEHAT uses white-hat deepfake algorithms to create 'self-deepfakes,' genuine portrait videos with the resemblance of the underlying identity, yet carry similar artifacts to deepfake videos; RDDP-SURROGATE employs surrogate functions (e.g., Gaussian noise) to process both genuine and forged examples, introducing equivalent noise, thereby sidestepping the need of deepfake algorithms. Towards detecting perfect deepfake videos that aligns with genuine ones, we present ID-Miner, a detector that identifies the puppeteer behind the disguise by focusing on motion over artifacts or appearances. As an identity-based detector, it authenticates videos by comparing them with reference footage. Equipped with the artifact-agnostic loss at frame-level and the identity-anchored loss at video-level, ID-Miner effectively singles out identity signals amidst distracting variations. Extensive experiments comparing ID-Miner with 12 baseline detectors under both conventional and RDDP evaluations with two deepfake datasets, along with additional qualitative studies, affirm the superiority of our method and the necessity for detectors designed to counter perfect deepfakes.

==> author_feedback/reviewer1.tex <==
\noindent\textbf{Responses to Reviewer \#1:} We are grateful for the review. The questions are clarified as follows.\\
\textbf{Choice of Deepfake algorithm $\mathcal{F}$.} We choose the First Order Motion Model as the deepfake algorithm $\mathcal{F}$ to train the artifact-agnostic encoder (Eq.~(2)).\\
\textbf{Requirements of deepfake algorithm $\mathcal{F}?$} ID-Miner can be adapted and trained for any deepfake algorithm that leverages the facial motions, where we test our framework among $11$ models, as shown in Tables 1 and 2. By substituting different subjects as the puppeteer and the victim, the artifact-agnostic loss can be constructed to guide ID-Miner to ignore the artifacts and focus on the underlying behavioral pattern.\\
\textbf{Details and reasons for GRU.} Concretely, we leverage a $2$ layer, bidirectional GRU with hidden state dimension $256$, which can overcome the gradient vanishing problem compared to vanilla RNN. Note that we choose GRUs (RNN-based models) over transformer-based models due to 1) their inference efficiency and 2) convergence speed. 


==> author_feedback/reviewer2.tex <==

\vspace{0.5mm}
\noindent\textbf{Responses to Reviewer \#2:} Thanks for the careful review. We address the weaknesses and the questions as follows.\\
\textbf{Cross-validation.} ID-Miner trained in VoxCeleb with Face Reenactment (FR) is directly validated on Celeb-DF with Faceswap (FS) in Table 2 due to its superior generalizability, while baselines are further cross-validated in Table 3 (see p.~5 ``Generalizability evaluation''). \\
\textbf{Reference dates.}  Out of the $12$ baselines, ID-Reveal (2021), FTCN (2021), EFNB4+SBIs (2022), ICT(2022), and TI2Net (2023) are recent (see p. 6 Table 1 and Table 2).\\
\textbf{Meaning of terms and symbols.} The term ``driving video'' denotes the input video that contains the sequence of facial motions ($\mathbf{a}$), which drives the resulting deepfake content. We provide the following description of videos consisting of sequential frames. In particular, $U$ and $V$ distinguish between deepfake content and real video recordings. $U(x,\mathbf{a})$ denotes deepfake with facial actions of $\mathbf{a}$ and appearance of $x$ (being changed from $s$ in the original $V(s,\mathbf{a})$). We use $\mathcal{F}_x\circ V$ to denote deepfake algorithm $\mathcal{F}$ operating on driving video $V$ with a facial appearance (portrait image) of $x$.
\\\textbf{Why the ethical concern?} The white-hat approach requires a fully functional deepfake algorithm. Thus, we are concerned that subsequent developments of RDDP-whitehat may spur improvement of deepfakes, e.g., those with fewer artifacts or can mimic victim behaviors, similar to the arms race of malware detection $[1]$.\\
$[1]$  Arms race in adversarial malware detection: A survey. ACM Computing Surveys (CSUR). 2021.\\
\textbf{Why only one $\lambda$.}  Ablation tests indicate the greater importance of the identity-anchored loss over the artifact-agnostic loss, and we thereby set $\lambda < 1$.\\
\textbf{Calculation of Avg. drop.} The drop is calculated by averaging the AUC scores over the five RDDP columns then comparing the average to the AUC scores under the conventional setting.\\
\textbf{Lower performances of ID-based baselines.} The lower performance may be due to the large number of identities in the experimented dataset, creating challenges to the ID-based detection models, which aim to model and differentiate between identity embeddings. Better performance can be attained by ID-based detectors if evaluated on a reduced set of identities.



==> author_feedback/reviewer3.tex <==
\newpage\noindent\textbf{Responses to Reviewer \#3:} Thank you for the kind review. We jointly address the weaknesses and questions as follows.\\
\textbf{Train baseline by RDDP-whitehat (R-white)?} Yes, ID-Miner will still beat the baseline. As shown in Tables 9 and 10 (p. 15) in the Supplementary, poor detection results for baselines trained under \textbf{R-white} underscores the need for ID-Miner, which handles the challenging RDDP.\\
\textbf{RDDP-surrogate (R-surr) vs model robustness?} The purpose of \textit{R-surr} is to drown out deepfake artifacts by global noise. Evidently, the non-ID-based baselines fail to pass the most basic model robustness setting. However, different from model robustness settings, which only perturbs the test examples, \textit{R-surr} applies noise equally to genuine (references) and the examined deepfakes, scrutinizing the reliance of ID-based baselines on artifacts.
 



==> author_feedback/reviewer4.tex <==
\vspace{0.5mm}
\noindent\textbf{Responses to Reviewer \#4:} We are grateful for the careful review. The questions are answered as follows.\\
\textbf{Technical contribution.} Unlike conventional contrastive learning, which mainly focuses on frame-to-frame comparison, we introduce a hierarchical objective, including both frame- and video-level comparison. Therefore, we can alleviate the misguidance from the artifact (frame-level) and extract robust action-based features  (video-level).\\
\textbf{Motivation and applicability of R-white.} We argue that conventional detection paradigms rely on the artifacts generated from current deepfake algorithms. Thus, \textit{R-white} is not designed to identify genuine faces but to create a hard example for deepfake detectors. By replacing genuine videos with reconstructed self-deepfakes (synthesized videos with the same identity), bridging the distribution gap from deepfakes (synthesized videos with a different identity) caused by artifacts. Real-world applications of \textit{R-white} include evaluation protocol for deepfake detectors and developing more robust adversarial training schemes, e.g., ID-Miner. The more robust detectors, in turn, provide preemptive protection against the emergence of advanced artifact-free deepfakes before their actual deployment.
% Utilizing \textit{R-white} enables the proactive development of detectors that do not rely on artifacts, anticipating the emergence of advanced deepfakes. For example, in critical election periods, if flawlessly executed deepfakes are strategically released, current detectors may fail to detect them, potentially causing political disruptions. \textit{R-white} provides a robust benchmark for detector development towards identifying artifact-free deepfakes prior to their actual deployment.
\\
\textbf{R-white vs. R-surr.} Both \textit{R-white} and \textit{R-surr} share the same objective: to eliminate the dependency on artifacts by creating a more demanding evaluation where genuine and fake videos are balanced to have similar distributions. \textit{R-white} accomplishes this by adjusting the distribution of genuine samples, while \textit{R-surr} achieves the same objective by transforming the distributions of both real and fake samples to a new domain.\\
\textbf{Advantage over ID-based schemes.} The main advantage of ID-Miner is its hierarchical structure and the pair of contrastive losses (Eq. (1)-(4) on p. 4), allowing ID-Miner to ignore artifacts and focus on robust features rooted in the facial action characteristics. Thus, as evident in the experiment comparisons (p. 6), ID-Miner functions without relying on deepfake imperfections under RDDP, serving as a preemptive countermeasure to future deepfake advancements.\\
\textbf{Conventional evaluation.}
We emphasize that the conventional evaluation is unreliable as it allows detectors to rely on artifacts. Evidently, prior works that optimized detecting artifacts find significant reductions under the more challenging RDDP (p. 6). Besides, the performance of ID-Miner is $0.85$ in terms of AUC score under the conventional protocol. 

==> table/ablation.tex <==
\begin{table}[t]\small
    \caption{\textbf{Different loss weight.} We vary the loss weight to investigate the effectiveness of \emph{artifact-agnostic loss}. The result is conducted on the Celeb-DF dataset.}
    \label{tab:ablation-lossweight}
    \centering
    \begin{tabular}{l c c cccc c}
        \toprule
        & \multirow{3}{*}{\shortstack[l]{\textsc{conven}\\ -\textsc{tional}}} 
        & \multirow{3}{*}{\shortstack[l]{RDDP-\\\textsc
        {whitehat}}} 
        & \multicolumn{4}{c}{\pcolsur} 
        & \multirow{2}{*}{\shortstack[l]{\\ \textit{avg. drop}}} \\
        \cmidrule(lr){4-7} 
        &                   & & Resize & JPEG & VC & GB \\
        
        \midrule
        $\lambda = 0$ & $0.896$ & $0.770$ & $0.781$ & $0.826$ & $0.795$ & $0.708$ & $-13.4\%$ \\
        $\lambda = 0.0001$ & $0.896$ &	$0.770$ & $0.781$ & $0.826$ & $0.795$ & $0.708$ & $-13.4\%$ \\
        $\lambda = 0.001$ & $0.896$	&$0.770$&	$0.781$&	$0.826$&	$0.795$&	$0.708$ & $-13.4\%$ \\
        $\lambda = 0.005$ & $0.860$	&$0.795$&	$0.799$&	$0.830$&	$0.801$	&$0.711$& $-8.5\%$ \\
        $\lambda = 0.0075$ & $0.859$&	$0.802$&	$0.799$&	$0.830$	&$0.817$&	$0.733$& $-7.3\%$ \\
        $\lambda = 0.01$ & $0.845$&	$0.808$&	$0.811$&	$0.832$&	$0.810$	&$0.720$& $-5.8\%$ \\
        $\lambda = 0.1$ &  $0.859$	&$0.823$&	$0.820$&	$0.832$&	$0.834$&	$0.743$& $-5.7\%$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> xapp/t_DFDCp.tex <==
\begin{table*}[t]\small
    \caption{\textbf{Evaluation on DFDCp (FS).}}
    \label{tab:DFDCp-FS}
    \centering
    \begin{tabular}{l c c cccc c}
        \toprule
        & \multirow{3}{*}{\shortstack[l]{\textsc{conven}\\ -\textsc{tional}}} 
        & \multirow{3}{*}{\shortstack[l]{RDDP-\\\textsc
        {whitehat}}} 
        & \multicolumn{4}{c}{\pcolsur} 
        & \multirow{2}{*}{\shortstack[l]{\\ \textit{avg. drop}}} \\
        \cmidrule(lr){4-7} 
        &                   & & Resize & JPEG & VC & GB \\

        \midrule
    Xception~\cite{chollet2017xception} & $\mathbf{0.}$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    MesoNet~\cite{afchar2018mesonet} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    FWA~\cite{li2018exposing} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    EfficientNet~\cite{tan2019efficientnet} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    Face X-ray~\cite{li2020face} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    FTCN~\cite{zheng2021exploring} & $0.$ & $0.$ & $\underline{0.}$ & $0.$ & $0.$ & $\mathbf{0.}$ & $-\%$ \\
    EFNB4+SBIs~\cite{shiohara2022detecting} & $\underline{0.}$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    ICT\cite{dong2022protecting} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$  \\
    TI2Net~\cite{liu2023ti2net} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    \midrule
    PWL~\cite{agarwal2019protecting} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    A\&B~\cite{agarwal2020detecting} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $\underline{-\%}$ \\
    ID-Reveal~\cite{idreveal2021cozzolino} & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $-\%$ \\
    \midrule
    \model & $0.$ & $\mathbf{0.}$ & $\mathbf{0.}$ & $\mathbf{0.}$ & $\mathbf{0.}$ & $\underline{0.}$ & $\mathbf{-\%}$  \\
    \model (no FLE) & $0.$ & $\underline{0.}$ & $0.$ & $\underline{0.}$ & $\underline{0.}$ & $0.$ & $-\%$ \\
        \bottomrule
    \end{tabular}
\end{table*}
